Temporally stable video segmentation without video annotations

Temporally consistent dense video annotations are scarce and hard to collect. In contrast, image segmentation datasets (and pre-trained models) are ubiquitous, and easier to label for any novel task. In this paper, we introduce a method to adapt still image segmentation models to video in an unsupervised manner, by using an optical flow-based consistency measure. To ensure that the inferred segmented videos appear more stable in practice, we verify that the consistency measure is well correlated with human judgement via a user study. Training a new multi-input multi-output decoder using this measure as a loss, together with a technique for refining current image segmentation datasets and a temporal weighted-guided filter, we observe stability improvements in the generated segmented videos with minimal loss of accuracy.

==> figures/CorrelationVsSmoothnessSigma.tex <==
\begin{figure}
\centering
    \includegraphics[width=0.6\linewidth]{figures/CorrelationVsSmoothnessSigma/sigmas.pdf}

  \caption{\textbf{Empirically calibrating the smoothness measure} sigma is the standard deviation for the Gaussian kernel, and r is the correlation with human judgement.}
  \label{fig:corrvssig}
\end{figure}


==> figures/training_refinement_consistency.tex <==
\begin{figure}
  \centering

\includegraphics[width=.7\linewidth, frame] {figures/ConsistencyVsN_inputs/placeholder.png} 
\caption{Fine-tuning a DeepLabV3 on a refined MS-COCO dataset improve the accuracy on the DAVIS video dataset. Also, starting from a refined model produces better results when adapted to video using our method.} 
\label{fig:training_refinement_consistency}
\end{figure}


==> figures/user_study.tex <==



% \begin{figure}
%   \centering

% \includegraphics[width=.48\linewidth] {figures/user_study/Median human score_log(Normalized inconsistency)_agreement_std_0.pdf} 
% \includegraphics[width=.48\linewidth] {figures/user_study/Median human score_log(Normalized inconsistency (Boundary))_agreement_std_1_no_ylabel.pdf}

% \vspace{0.2cm}     


% \includegraphics[width=.48\linewidth] {figures/user_study/Median human score_log(Unnormalized inconsistency)_agreement_std_0.pdf} 
% \includegraphics[width=.48\linewidth] {figures/user_study/Median human score_log(Smoothness)_agreement_std_0 (1).pdf}

% \caption{***Preliminary figures, Nadav will take over this part*** Our consistency measure is correlated with human judgment. Top left: all the data. Top right: only videos with high agreement between humans. Bottom left: Unnormalized measure has a inferior correlation with human judgment. Bottom right: Smoothness does not capture human's notion of inconsistency. r stands for Pearson correlation.} 
% \label{fig:user_study}
% \end{figure}




==> stuff/03_5_limitations.tex <==
%moved to the conclusions section

==> stuff/03_method.tex <==
\section{Consistency Measures for Video Segmentation}
\label{sec:consistency_measures}

% \subsection{Definitions}
% \label{sec:definitions}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/measures/measures-crop.pdf}
    \caption{\textbf{Various quality measures for video segmentation.} We consider two video frames (top left), with various possible segmentations of a salient object (the star). In the best case scenario of high \emph{accuracy} (top right), the object is segmented precisely at all frames. In the case of low accuracy, we can look at a) the degree of \emph{consistency}, how well the mask is following the relative motion of the object (bottom left), or b) the degree of \emph{smoothness}, how much the mask itself is changing between frames (bottom right).}
    \label{fig:measures}
\end{figure}

Most of us have an intuitive grasp of what it means for a video object segmentation to be temporally consistent. Our first step in improving consistency was to quantify that intuition. To measure the perceived segmentation consistency, we first wanted to find a metric we can calculate automatically and correlates highly with human perception, hopefully one that can be implemented as a loss in a learning based algorithm.

There are two main approaches to measure temporal consistency. The first one is based on quantifying high frequencies in the temporal domain. A typical representative of this approach is the following \emph{smoothness measure}, as presented by Eilertsen et al.~\cite{eilertsen2019single}: 
%
\begin{equation}
E_{smooth}(\{O_t\}_{t=1}^T) = \sum_t\lVert O_t - G_\sigma(O_t)\rVert_2 / N_{bd}
\end{equation}
%
%
% \begin{equation}
% E_{smooth}(O)_{i,j,t} = |O_{i,j,t} - (G_\sigma(O))_{i,j,t}|^2\ 
% \end{equation}
%
where $O_t$ is the segmentation at time $t$, $N_{bd}$ is the number of pixels on object boundaries, and $G_\sigma$ is a Gaussian blur performed in the temporal dimension $t$. The parameter $\sigma$ is selected to be 0.15 seconds (which as about 5 frames for 30fps video) as described in Eilertsen et al.~\cite{eilertsen2019single}. We verified in our user study (in \Cref{sec:user_study_results}) that for YouTubeVOS videos the sigma with highest agreement with humans is about 0.15 seconds, which corresponds to about 1 frame, since YouTubeVOS is annotated with masks at about 6fps. This is in agreement with theory about optimal sigma \cite{laird2006spatio}. We generalize this measure to the multi label segmentation task, by smoothing each class independently with $G_\sigma$ and merging the results with $\textrm{argmax}$. Intuitively, a segmentation mask with higher jitter will score higher (worse) on this measure. Consequently, this measure tends to prefer highly blurred masks, even at the expense of accuracy \aharon{consistency also doesn't care about accuracy.} (Figure \ref{fig:smoothing_baseline}). 
% Furthermore, in situations where the motion in the video is fast and not rigid, smoothness can simply be an inadequate measure of consistency: for each pixel, temporal smoothing can have two outcomes, either it propagates a part of the mask that corresponds to the same part in the object, or it propagates some other part to the same location because of rigid and non rigid motion of objects.  \tavi{i don't understand this, how can smoothness harm consistency? isn't it a measure?} In the latter case, smoothing harms consistency in the sense of a false registration between segmentations of similar object parts (Fig.~\ref{fig:consistency_vs_smoothness}).

For the aforementioned reasons, the second canonical approach uses optical flow calculation and warping, despite its computational cost, to track pixels to their target location, and verify that the segmentation remains consistent between origin and target. Therefore, it obviates the need to search for the best value of $\sigma$. The quality of the optical flow is crucial for the end result of our method, hence we use GMA \cite{jiang2021learning}, a state-of-the-art deep optical flow method. On the other hand, unlike smoothness based measures, flow based measures have the drawback of not covering occluded pixels. Such occluded pixels are identified by doing a forward-backward consistency check of the optical flow \cite{sundaram2010dense, ruder2016artistic}.
% \begin{equation}
% M_{I_{t}\xrightarrow{}I_{t+1}} =
% \begin{cases}
%     1,& \|I_{t} - W_{I_t\xrightarrow{}I_{t+1}}(W_{I_{t+1}\xrightarrow{}I_{t}}(I_t))\|_1 > \tau \\
%     0,& \text{otherwise}
% \end{cases}
% \end{equation}
% Where $I_t$ is the video frame at time $t$, $W$ is the warping function based on the optical flow between the frames. We choose the thresh to be equal to 10, where $I_t$ is between 0 and 255.
% This is different than the approach taken in \cite{ruder2016artistic}, where the valid pixels are chosen based on warping and back-warping the flow field itself, choosing only pixels that returned to a similar location. This is assuming that the optical flow is perfect, and not taking into account violations of the constant brightness assumption. On the other hand, our approach bypass this limitation by choosing only pixels with similar brightness level.
Based on these optical flow and occlusion detection algorithms, we follow \cite{ruder2016artistic} in defining our \emph{optical flow-based consistency measure}. Our raw data is in the form of images (frames) $I_t$ together with the corresponding multi-class segmentations $O_t$. The segmentations are encoded in categorical form, that is each pixel is associated with a label $n\in\{0,\ldots,L\}$ where $L$ is the total number of classes. First we define a pair-wise symmetric discrepancy measure between two image-segmentation pairs:
% \begin{equation}
% \begin{aligned}
% & E_{pair}((I_p,O_p),(I_q,O_q)) = \\
% & \frac{1}{\sum{M_{I_t\xrightarrow{}I_{t+1}}}}  \sum_{i=1}^{N}{M_{I_{t}\xrightarrow{}I_{t+1}}} \|O_{t+1} - W_{I_t\xrightarrow{}I_{t+1}}(O_t)\|_1
% \end{aligned}
% \end{equation}
\begin{multline}
\label{eq:pairwise_loss}
E_{pair}((I_p,O_p),(I_q,O_q)) =\\
\lVert M_{I_p\rightarrow I_q}\cdot d_{cat}(O_q, W_{I_p\rightarrow I_q}(O_p))\rVert_1 \Big/ \lVert M_{I_p\rightarrow I_q}\rVert_1+\\
\lVert M_{I_q\rightarrow I_p}\cdot d_{cat}(O_p, W_{I_q\rightarrow I_p}(O_q))\rVert_1 \Big/ \lVert M_{I_q\rightarrow I_p}\rVert_1
\end{multline}
where $W_{I\rightarrow I'}$ denotes the optical-flow derived warp between two images $I,I'$, and $M_{I\rightarrow I'}$ denotes the associated binary occlusion mask (0 for occluded pixels, 1 for non-occluded). The categorical distance $d_{cat}(\cdot,\cdot)$ takes the value 1 at pixels with the same label in both segmentations and 0 otherwise. The total measure for a video is calculated then by considering the pair-wise consistency between all pairs of frames within a temporal window of size $K$: 
\begin{multline}\label{eq:Econs}
E_{cons}(\{(I_t,O_t)\}_{t=1}^{T}) =\\
\frac{1}{N}\frac{1}{\text{TK}} \sum_{|i-j|\leq K} E_{pair}((I_i,O_i),(I_j,O_j))
\end{multline}
where $N$ is a suitable normalization constant, to be discussed below. We use $K=3$, for a total window size $2K+1=7$, by default, see Sec.~\ref{sec:decoder_training} for further discussion on the window size.

% \subsection{Normalizing the consistency measure}
% \label{sec:normalization}

As the measure \eqref{eq:Econs} is an average over all pixels (and not a relative measure, since we don't have a reference), it might suffer from spurious correlations with the size of the non-background objects in the masks (Fig. \ref{fig:consistency_Vs_object_size}). The reasoning is that it is easier to be consistent for background pixels. Furthermore, we presume that the major source of inconsistencies reside in the boundaries between objects (or between an object and the background). Thus, we hypothesized that normalizing the consistency measure by a scalar $N$ that is proportional to the object perimeter should be done. Indeed, normalizing the consistency measure with $N=\sqrt{N_{nbg}}$, the square root of the number of non-background pixels (that is pixels that belong to any segmentation class other than 'background'), eliminates most of the correlation with the object size (Fig.~\ref{fig:consistency_Vs_object_size}).
Because objects are often not simple geometrical shapes, their boundary might be of a fractal dimension different than 1. For that reason, instead of estimating the length of the boundaries as $N_{nbg}^{1/2}$, we counted the actual number $N_{bd}$ of pixels on the boundary of objects and normalized with $N=N_{bd}$ which further reduced the spurious correlation with object size. Furthermore, this kind of normalization slightly improved the correlation of this measure with human intuition (see Section \ref{sec:user_study_results}).

% we experimented with raising it to the power of $k/2$, where k is a real number that should correspond to the characteristic fractal dimension of real objects. We also calculate the mean empirical Minkowski–Bouligand dimension for every one of the 1000 videos we tested. We show that the fractal dimension of real objects can be well approximated by 1, and when calculating it for each video separately, one gets a negligible improvement.

\input{figures/consistency_Vs_object_size}

To better illustrate the conceptual difference between smoothness and consistency, we show in \Cref{fig:consistency_vs_smoothness} slices in space-time from two different videos, with corresponding human-annotated segmentation masks. We then align each of the videos to one of its frames using optical flow, and compute the consistency score based on the flow. We also compute the consistency score on the original video. Despite some imperfections in the flow computation, the consistency score that is derived from it matches human intuition, as the human annotated mask of the pangolin is qualitatively much more jittery than the one of the bear (we include both videos in the supplementary material). The smoothness measure, however, shows inverse relation in the case of these two videos, since the bear moves a significant distance while having a precise annotation, whereas the pangolin shows smaller motion, but its annotation is more jittery.

\input{figures/consistency_vs_smoothness}

\section{User Study of Measured vs Perceived Consistency}

\subsection{Experimental setup}

We designed a user study to verify that our proposed consistency measure is well aligned with the human perception of consistency, by asking crowd workers to rank the consistency of the segmentation masks of $96$ videos on a Likert scale of 1-5. We paid the workers \$0.24 per labeling job and collected nine rankings for each video.

In setting up the study, we noticed that some participants tend to mix-up the concepts of consistency and accuracy. That is, they ranked the \emph{accuracy} of the segmentation masks instead of their \emph{consistency}. To mitigate the problem, we introduced ``qualification videos'' into the experiment. To construct a qualification video, we select a clip with an accurate ground-truth segmentation mask, and corrupt the mask along two separate axes -- accuracy and consistency. To corrupt the accuracy we erode $n$ pixels from the mask in a random direction, where $n$ is in $\{0, 10, 20\}$. To corrupt the consistency of the mask we use a randomly chosen local piecewise-affine transformation, where the displacement magnitude for each pixel is randomly drawn from $\{0, 4, 8\}$ and the displacement direction is randomly chosen. Calculating the two measures for the corrupted set of videos, we verified that the transformations had the intended effect. After corrupting the original video along the two axes we get a $3\times3$ grid of corrupted clips, where each clip in the grid has an accuracy rank and a consistency rank, each on a scale of 1-3. Overall, we introduced $4 \cdot 9=36$ qualification videos to the user study. Our expectation is that the ranking of crowd workers that correctly distinguish between consistency and accuracy (i.e., understand the task) should have high correlation with the \emph{consistency} value of the qualification videos, but low correlation with the \emph{accuracy} value of the videos. In contrast, the ranking of crowd workers that confuse the concepts of consistency and accuracy should have high correlation with accuracy value of the qualification videos. 

Filtering out the responses of crowd workers whose ranking of the qualification videos had higher correlation with the accuracy value of the videos than with the consistency value of the videos, the average ranking was $2.65$ and the average standard deviation for each video was $1.08$. The agreement between the qualifying workers was acceptable for such a subjective task, with mean pairwise Spearman correlation of $0.38$. We aggregated the nine 1-5 labels for each video by taking their mean.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.35\textwidth]{media/video_grid.jpeg}
%     \caption{video grid. \nnote{Just in case, we probably shouldn't keep it}}
%     \label{fig:video_grid}
% \end{figure}

\subsection{Results}
\label{sec:user_study_results}

As can be seen in Figure \ref{fig:user_study_inconsistency}, the proposed consistency measurement is relatively well aligned with the human rankings of consistency, reaching a Spearman correlation of $0.569$ (p-value=$1.5\mathrm{e}{-9}$). 

\begin{figure}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/user_study/Mean human score_Inconsistency (log scale)_agreement_std_0 (1).pdf}
    \label{fig:user_study_inconsistency_all}
  \end{subfigure}
  %
  \quad
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/user_study/Mean human score_Smoothness (log scale)_agreement_std_0 (1).pdf}
    \label{fig:user_study_smoothness_all}
  \end{subfigure}
    \quad
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/user_study/smoothnessVsConsistency.pdf}
    \label{fig:user_study_smoothness_vs_consistency}
  \end{subfigure}
      \quad
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figures/CorrelationVsSmoothnessSigma/sigmas.pdf}
    \label{fig:user_study_smoothness_all_sigmas}
  \end{subfigure}
  \caption{\textbf{User study.} The smoothness and consistency measures are not perfectly correlated (bottom left). The top subfigures show that our consistency measure (left) is better correlated with human judgment of consistency relative to the smoothness measure (right) \cite{eilertsen2019single}. The standard deviation for the smoothness measure was chosen to maximize the correlation with humans (bottom right). Videos where taken from the YouTubeVOS dataset.}
  \label{fig:user_study_inconsistency}
\end{figure}

However, our user study demonstrates that the smoothness measure captures the human notion of consistency to a lesser extent. Indeed, as can be seen in Figure \ref{fig:user_study_inconsistency}, this measurement is less correlated with the rankings of crowd workers, having a lower Spearman correlation of $0.474$ (p-value=$1.08\mathrm{e}{-6}$)).


% \begin{figure}
%   \begin{subfigure}[t]{0.22\textwidth}
%     \includegraphics[width=\textwidth]{figures/user_study/Mean human score - inconsistency - agg_ True.pdf}
%     \caption{Ours}
%     \label{fig:user_study_inconsistency_high_agg}
%   \end{subfigure}
%   %
%   \quad
%   \begin{subfigure}[t]{0.22\textwidth}
%     \includegraphics[width=\textwidth]{figures/user_study/Mean human score - smoothness - agg_ True.pdf}
%     \caption{Smoothness measure}
%     \label{fig:user_study_smoothness_high_agg}
%   \end{subfigure}
%   \caption{Removing low-agreement videos drastically improves the correlation of our inconsistency measurement with human rankings, but not the correlation of the ``smoothness measure''.}
%   \label{fig:user_study_smoothness}
% \end{figure}





We were also interested in verifying that the normalization method described in Section \ref{sec:consistency_measures} indeed improves the correlation of the inconsistency measure with human intuition of consistency. As expected, The correlation between the non-normalized version of the inconsistency measure and the human rankings was a bit lower (Spearman corr=$0.535$, p-value=$1.9\mathrm{e}{-8}$).

% \subsection{A note about low-agreement videos}

% As the task of evaluating the consistency of segmentation masks is highly subjective, we investigated the performance of the measurement on the subset of videos that the participants had reached high agreement on. The reasoning for that is that disagreement between crowd workers can have two explanations: 1) they did not understand the task or paid attention, or 2) consistency is a matter of opinion in this specific video. Either way, these examples are above the precision level that our user study can provide, and thus introduce noise to the overall experiment. To test this hypothesis, we inspected a random sample of low-agreement videos (we consider a video to have low agreement if the standard deviation of its nine rankings is higher than $1.0$). We noticed that in many cases the masks in those videos were relatively consistent on most parts of the segmented object, but very inconsistent in a specific region of the object or in specific frames. Therefore, a possible explanation for the low agreement in those videos is that some labelers decided to focus on the sections of low consistency, while others decided to give more weight to the consistent parts (or, in other words, the crowd workers had different opinions as to how a consistent video should look like). 

Given the subjective nature of the task, it is not unexpected that the participants might fail to reach consensus in their rankings for some of the videos. We inspected a random sample of such low-agreement videos (standard deviation of the nine rankings higher than $1.0$), to better understand their effect on the results of the study. We noticed that in many cases the masks in those videos were relatively consistent over the majority of the segmented object, but very inconsistent in a specific region of the object or in specific frames. Therefore, a possible explanation for the low agreement in those videos is that some participants tend to focus on the occasional artifacts, while others tend to rate the overall consistency; a difference of opinion in what constitutes a 'consistent' video. Removing the low-agreement videos from the sample, the correlation between our consistency measure and human rankings increases to $0.724$ (p-value=$1.3\mathrm{e}{-6}$). This trend apply also to the smoothness measure -- removing low-agreement videos improves its correlation score to $0.671$ (p-value=$1.39\mathrm{e}{-5}$).

\section{Training Temporally Consistent Segmentation Models}

\subsection{A Multi-input Decoder Architecture for Segmentation}
\label{sec:decoder_training}

Intuitively, the temporal consistency of video segmentation can benefit with the access to information from multiple frames. However, it is not clear how to incorporate such information. Towards this end, we propose a modification of the popular DeepLabV3 \cite{chen2017rethinking} decoder to process multiple frames by increasing the number of input and output channels (Fig.~\ref{fig:pipeline}). We decided to do this modification only to the decoder as it is more computationally efficient.

% \orestis{Might move or rewrite this, not super clear as is.}
% Given a set of encoded input frames ${Encoder(I)}_t^T$ and inconsistent masks ${Encoder(N)}_t^T$, we train a decoder to output masks that minimize our consistency loss on non-occluded pixels, and to stay close to ${N}_t^T$ in occluded pixels. This defines an intractable non-convex optimization problem.

We use a standard DeepLabV3 encoder with a ResNet50 backbone to encode the frames and the segmentation outputs from an off-the-shelf DeepLabV3 segmentation model. On top of these encoded representations, we train a multi-input multi-output decoder to predict the delta from the prediction of the baseline decoder. During training, we pass randomly chosen sets of input frames to the encoder, and we minimise the mean of the pair-wise consistency loss \eqref{eq:pairwise_loss} over every pair of input frames. We use the Adam optimizer and a learning rate of $10^{-5}$. The training code is publicly available.

A larger number of input frames has the advantage of providing a larger set of non-occluded pixels, as an occluded pixel in one frame might be non-occluded in another. Moreover, it can provide multiple votes for every non-occluded pixel, correcting for some warping errors. However, increasing the number of inputs is computationally expensive, as it increases the number of optical flow computations during training quadratically, and also makes inference slower. For our experiments we used 7 input frames; see Fig.~\ref{fig:ConsistencyVsN_inputs} for the effect of different number of input frames. 

% As our method rely on a costly pairwise optical flow calculation, it should be justifiable to use a larger temporal context. Also, because our method only uses non-ocluded pixels to compute the consistency loss, adding more input frames should only improve both accuracy and consistency. Empirically, this is indeed the case (Fig. \ref{fig:ConsistencyVsN_inputs}).

\input{figures/ConsistencyVsN_inputs}

\subsection{A Refined Image Segmentation Dataset}

The quality of the initial encoder affects the quality of our multi-input decoder, regardless of temporal consistency. To improve the encoder quality, we tested whether training it on a refined version of MS-COCO \cite{lin2014microsoft} will result in better segmentation masks and a better encoder. We used the latest Cascade-PSP \cite{cheng2020cascadepsp} to create a refined version of MS-COCO, with mask edges that are more closely aligned to object boundaries (Fig. \ref{fig:YoutubeVOS_refinement_consistency}). Note that such refinement procedures are too computationally intensive for use during inference.

We observed that training DeepLabV3 on such a refined version of MS-COCO improves temporal consistency on the DAVIS dataset, and slightly improves IoU score on a subset of 500 relabelled PascalVOC examples \cite{cheng2020cascadepsp}  (Table \ref{tab:main}). However, training on a refined dataset slightly decreases the recall on DAVIS. We believe that this is caused by the fact that the refinement method we used (Cascade-PSP) has a tendency to drop small, background objects. Regardless, this result means that the network is prone to learning the labelling errors in the training dataset, and therefore improving labelling quality can have a substantial effect on temporal consistency when shifting the domain to video segmentation (Fig.~\ref{fig:YoutubeVOS_refinement_consistency}).

\input{figures/YoutubeVOS_refinement_consistency}

% For reasons of resource optimization, image and video segmentation datasets often contain labelling errors. 
% Training deep neural networks on labelling errors may result in two outcomes: 1) the networks will learn to ignore the errors. 2) the networks will learn a smoother function to maximally account for these labelling errors.
% We show that some portion of temporal inconsistencies can be improved merely by a post-processing that 
% Outputs from image segmentation models can also be refined to produce edge aligned masks. However, refinement procedures can be computationally intensive and are not practical to use during inference. 

\subsection{Benchmarks}
\label{sec:benchmarks}
\orestis{Copy-pasted, needs editing}

The basic result is that optimizing a multi-input decoder with our consistency loss on DeepLabV3 representations of DAVIS video frames substantially improve temporal stability with a minor drop in recall (Table \ref{tab:main}). \orestis{What is 'naive'? What is 'TI'?}

\input{tables/main_result.tex}

Notice that we are unable to use the IoU measure when switching the domain from images to videos. This is because the set of classes between the domains is different from MS-COCO and DAVIS. As an alternative, we use only the recall measure, which gives an estimate for the segmentation quality on object classes that are shared between the two domains. We do measure IoU on images when the model remains a single-input model, and show that the IoU levels there are not degrading.

Interestingly, when we start optimizing our multi-input decoder from representations of an encoder trained on refined MS-COCO (Table \ref{tab:main}, last row), we get a better consistency at the price of a lower recall levels. This is due to the tendency of the refinement network \cite{cheng2020cascadepsp} to undersegment, especially for small, background objects. This may be desirable if one is interested on segmenting the main object in the video and values stability over accuracy.

% \subsubsection{Baseline: temporally smoothing}
The most basic baseline one should compare to is a Gaussian blur in the temporal dimension. This form of temporal smoothing can improve the consistency of video segmentation. However, improving consistency should never stand without accuracy, as one can always return the trivial solution of a constant mask. So a crucial question to ask is whether our method provides a solution that is outside the consistency-accuracy Pareto front of temporal smoothing. As shown in \ref{fig:smoothing_baseline}, smoothing doesn't necessarily improves consistency, and monotonously degrades accuracy. In contrast, our method shows that one can improve temporal consistency without loosing accuracy.

\input{figures/smoothing_baseline}

\subsection{Postprocessing with 3D guided filter}
\label{sec:guided_filter}

To improve consistency further we experimented with post processing with guided filter\cite{he2012guided}, extended to 3D (2D+time), with the expectation that such a local filter will further improve the agreement between model predictions on consecutive frames. In particular, we implemented the weighted guided filter of~\cite{liba2020sky}, which assigns a smaller weight to low confidence pixels. We extend it to 3D in a straightforward manner, by stacking the output masks as a volume and using the stack of frames as the guide, a process that takes a few seconds for a short clip. For multi-class predictions, we filter each mask independently, after softmax but before binarization, and set the label of a pixel to the class with highest value after filtering.

The effect of applying the 3D weighted guided filter (WGF) is summarized in \Cref{tab:guidedfilt}. This additional post processing step improves consistency significantly. It also shows small improvements in smoothness, although guided filters usually tend to sharpen, so we attribute this improvement to the masks being more consistent. This improved consistency comes with a price of degraded recall. When we apply the WGF with temporal kernel size equal to 1, which is effectively a 2D WGF, it has negligible effect on consistency and smoothness (but slightly better recall). This demonstrates the effectiveness of applying the filter on the temporal dimension as well.

\input{tables/guidedfilt}

\subsection{Temporal consistency for models trained on video}
Having shown in detail how an image segmentation model can be turned into a temporally stable video model, we briefly turn to the question of temporal stability in models that were trained on video data. We tested the straight-forward approach of fine-tuning a video model on the same data it was originally trained on (without additional data), but adding our proposed consistency loss. Starting from a state-of-the-art video segmentation model \cite{mahadevan2020making} and training as described above, one can get a variety of possible solutions. In particular, here we show that one can explore the accuracy-consistency trade-off by changing the number of training epochs \Cref{fig:video_seg}. We leave for future work the attempt to improve video segmentation models without access to the original labeled video data by using a teacher student approach with our consistency loss (as we showed in section \ref{sec:decoder_training}).

\input{figures/video_seg.tex}

==> stuff/04_experiments.tex <==
\section{Experiments}
\orestis{OK, I think everything here can be moved into the previous sections, and we can get rid of this section completely.}

% \subsection{Mask Refinement}
% \orestis{I moved this into section 5}


% \subsection{User Study}

% \input{figures/user_study}

% \nnote{to do?}
% \orestis{Maybe we better keep all the user study material in one section?}


\subsection{Multi-Input decoder}
\orestis{Planning to also move this into the main text in the morning.}

The basic result is that optimizing a multi-input decoder with our consistency loss on DeepLabV3 representations of DAVIS video frames substantially improve temporal stability with a minor drop in recall (Table \ref{tab:main}). \orestis{What is 'naive'? What is 'TI'?}

\input{tables/main_result.tex}

Notice that we are unable to use the IoU measure when switching the domain from images to videos. This is because the set of classes between the domains is different from MS-COCO and DAVIS. As an alternative, we use only the recall measure, which gives an estimate for the segmentation quality on object classes that are shared between the two domains. We do measure IoU on images when the model remains a single-input model, and show that the IoU levels there are not degrading.

Interestingly, when we start optimizing our multi-input decoder from representations of an encoder trained on refined MS-COCO (Table \ref{tab:main}, last row), we get a better consistency at the price of a lower recall levels. This is due to the tendency of the refinement network \cite{cheng2020cascadepsp} to undersegment, especially for small, background objects. This may be desirable if one is interested on segmenting the main object in the video and values stability over accuracy.






\subsubsection{Baseline: temporally smoothing}
The most basic baseline one should compare to is a Gaussian blur in the temporal dimension. This form of temporal smoothing can improve the consistency of video segmentation. However, improving consistency should never stand without accuracy, as one can always return the trivial solution of a constant mask. So a crucial question to ask is whether our method provides a solution that is outside the consistency-accuracy Pareto front of temporal smoothing. As shown in \ref{fig:smoothing_baseline}, smoothing doesn't necessarily improves consistency, and monotonously degrades accuracy. In contrast, our method shows that one can improve temporal consistency without loosing accuracy.


\input{figures/smoothing_baseline}


% \subsubsection{The effect of temporal context size}
% \orestis{Pulling this back into section 5.1}
% As our method rely on a costly pairwise optical flow calculation, it should be justifiable to use a larger temporal context. Also, because our method only uses non-ocluded pixels to compute the consistency loss, adding more input frames should only improve both accuracy and consistency. Empirically, this is indeed the case (Fig. \ref{fig:ConsistencyVsN_inputs}).


% \input{figures/ConsistencyVsN_inputs}



% \subsection{Improving video models' temporal consistency}
% \orestis{moved to end of sec 5}
% \orestis{This looks incomplete.}
% We have shown that any image segmentation model can be turned into a temporally stable video model. In this section, we explore temporal stability in models that were trained on video data. We do so by fine-tunning a video model on the same data it was originally trained on (without additional data), but with an additional consistency loss. 
% Starting from a state-of-the-art video segmentation model \cite{mahadevan2020making} and training as described above, one can get a variety of possible solutions. In particular, here we show that one can explore the accuracy-consistency tradeoff by changing the number of training epochs \ref{fig:video_seg}.

% \input{figures/video_seg.tex}


% \subsection{3D guided filter}
% \orestis{To fold into sec 5}
% The effect of applying 3D Weighted Guided Filter is summarized in \Cref{tab:guidedfilt}. This additional post processing step improves consistency significantly. It also shows small improvement in smoothness, although Guided Filter usually tends to sharpen, so we attribute this improvement to the masks being more consistent. This improved consistency comes with a price of degraded recall. When we apply WGF with temporal kernel size equal to 1, which is effectively a 2D WGF, it has negligible effect on consistency and smoothness (but slightly better recall). This demonstrates the effectiveness of applying the filter on the temporal dimension as well.

% \input{tables/guidedfilt}







==> stuff/04_experiments_OLD.tex <==
\section{Experiments}

\vspace{-.13cm}\boldparagraphnovspace{Datasets} We report results on commonly-used single-object datasets \textit{Chairs}~\cite{Oechsle2020THREEDV}, \textit{Cats}~\cite{Zhang2003ICCV}, \textit{CelebA}~\cite{Liu2015ICCV}, and \textit{CelebA-HQ}~\cite{Karras2018ICLR}.
The first consists of synthetic renderings of Photoshape~chairs~\cite{Park2018ACM}, and the others are image collections of cat and human faces, respectively.
The data complexity is limited as the background is purely white or only takes up a small part of the image. 
We further report results on the more challenging single-object, real-world datasets \textit{CompCars}~\cite{Yang2015CVPR}, \textit{LSUN Churches}~\cite{Yu2015ARXIV}, and \textit{FFHQ}~\cite{Karras2019CVPR}.
For \textit{CompCars}, we randomly crop the images to achieve more variety of the object's position in the image.\footnote{\noindent We do not apply random cropping for \cite{Henzler2019ICCV} and \cite{Schwarz2020NEURIPS} as we find that they cannot handle scenes with non-centered objects (see supplementary).}
For these datasets, disentangling objects is more complex as the object is not always in the center and the background is more cluttered and takes up a larger part of the image.
To test our model on multi-object scenes, we use the script from~\cite{Johnson2017CVPR} to render scenes with $2$, $3$, $4$, or $5$ random primitives (\textit{Clevr-N}).
To test our model on scenes with a varying number of objects, we also run our model on the union of them ($\textit{Clevr-2345}$).

\boldparagraph{Baselines} We compare against voxel-based PlatonicGAN~\cite{Henzler2019ICCV}, BlockGAN~\cite{Nguyen-Phuoc2020NEURIPSp}, and HoloGAN~\cite{Nguyen-Phuoc2019ICCV}, and radiance field-based GRAF~\cite{Schwarz2020NEURIPS} (see~\secref{sec:rel-work} for a discussion of the methods).
We further compare against HoloGAN w/o 3D~Conv, a variant of~\cite{Nguyen-Phuoc2019ICCV} proposed in~\cite{Schwarz2020NEURIPS} for higher resolutions.
We additionally report a ResNet-based~\cite{He2016CVPR} 2D~GAN~\cite{Mescheder2018ICML} for reference.

\boldparagraph{Metrics} We report the Frechet Inception Distance (FID) score~\cite{Heusel2017NIPS} to quantify image quality.
We use \num{20000} real and fake samples to calculate the FID score.

\subsection{Controllable Scene Generation}
\begin{figure}
  \centering
  \input{tables/table_decomposition.tex}
  \vspaceunderfig%
  \caption{
      \textbf{Scene Disentanglement.}
      From top to bottom, we show only backgrounds, only objects, color-coded object alpha maps, and the final synthesized images at $64^2$ pixel resolution.
      Disentanglement emerges without supervision, and the model learns to generate plausible backgrounds although the training data only contains images with objects.
      }
  \label{fig:disentanglement}
\end{figure}
\begin{figure}
  \includegraphics[width=1.\linewidth]{gfx/experiments/progression/clevr_progression}
  \vspaceunderfigext%
  \caption{
      \textbf{Training Progression.}
          We show renderings of our model on \textit{Clevr-2345} at $256^2$ pixels after $0$, $1$, $2$, $3$, $10$, and $100$-thousand iterations.
          Unsupervised disentanglement emerges already at the very beginning of training.
      }
  \label{fig:training-progression}
\end{figure}
\begin{figure*}
  \centering
  \begin{subfigure}[t]{.495\linewidth}
      \centering\includegraphics[width=\linewidth]{gfx/experiments/cars/256/ours/rotation}\vspace{-.1cm}
      \subcaption{Object Rotation}
      \label{subfig:control-elevation}
  \end{subfigure}
  \begin{subfigure}[t]{0.495\linewidth}
      \centering\includegraphics[width=\linewidth]{gfx/experiments/cars/256/ours/elevation}\vspace{-.1cm}
      \subcaption{Camera Elevation}
      \label{subfig:control-rotation}
    \end{subfigure}
    \begin{subfigure}[t]{1.\linewidth}
        \centering\includegraphics[width=0.495\linewidth]{gfx/experiments/cars/256/ours/change_appearance}
        \includegraphics[width=0.495\linewidth]{gfx/experiments/ffhq/256/ours/change_appearance}
        \label{subfig:control-appearance}\vspace{-.1cm}
        \subcaption{Object Appearance}
      \end{subfigure}
      \begin{subfigure}[t]{.495\linewidth}
          \centering\includegraphics[width=\linewidth]{gfx/experiments/cars/256/ours/translate_x}\vspace{-.1cm}
          \subcaption{Depth Translation}
          \end{subfigure}
        \begin{subfigure}[t]{.495\linewidth}
            \centering\includegraphics[width=\linewidth]{gfx/experiments/cars/256/ours/translate_y}\vspace{-.1cm}
            \subcaption{Horizontal Translation}
           \end{subfigure}
        \begin{subfigure}[t]{1.\linewidth}
            \centering\includegraphics[width=\linewidth]{gfx/experiments/clevr2/256/ours/translation_circle2}\vspace{-.1cm}
            \subcaption{Circular Translation of One Object Around Another Object}
            \label{subfig:control-circle}
          \end{subfigure}
  \vspaceunderfig\vspace{-.1cm}
  \caption{
      \textbf{Controllable Scene Generation at $256^2$ Pixel Resolution.} 
      Controlling the generated scenes during image synthesis: Here we rotate or translate objects, change their appearances, and perform complex operations like circular translations.
      }
      \vspace{-.3cm}
  \label{fig:controllable-scene-gen}
\end{figure*}
\begin{figure} 
  \centering
  \begin{subfigure}[t]{1.\linewidth}
  \includegraphics[width=1.\linewidth]{gfx/experiments/cars/256/ours/translate_x_increase}\vspace{-.1cm}
    \subcaption{Increase Depth Translation}
    \label{subfig:increase-z-translation}
\end{subfigure}
  \begin{subfigure}[t]{1.\linewidth}
  \includegraphics[width=1.\linewidth]{gfx/experiments/cars/256/ours/translate_y_increase}\vspace{-.1cm}
    \subcaption{Increase Horizontal Translation}
    \label{subfig:increase-z-translation}
\end{subfigure}
  \begin{subfigure}[t]{1.\linewidth}
  \includegraphics[width=1.\linewidth]{gfx/experiments/clevr2/256/ours/add_object_ext}\vspace{-.1cm}
\subcaption{Add Additional Objects (Trained on Two-Object Scenes)}  
\label{subfig:add-object}
\end{subfigure}
\begin{subfigure}[t]{1.\linewidth}
  \includegraphics[width=1.\linewidth]{gfx/experiments/cars/256/ours/add_object_ext}\vspace{-.1cm}
\subcaption{Add Additional Objects (Trained on Single-Object Scenes)}  
\label{subfig:add-object}
\end{subfigure}
  \vspaceunderfig\vspace{-.1cm}
  \caption{
      \textbf{Generalization Beyond Training Data.}
      As individual objects are correctly disentangled, our model allows for generating out of distribution samples at test time.
      For example, we can increase the translation ranges or add more objects than there were present in the training data.
      }
  \label{fig:generalization}
\end{figure}
\vspace{-.13cm}\boldparagraphnovspace{Disentangled Scene Generation} 
We first analyze to which degree our model learns to generate disentangled scene representations. 
In particular, we are interested if objects are disentangled from the background.
Towards this goal, we exploit the fact that our composition operator is a simple addition operation (Eq.~\ref{eq:composition}) and render individual components and object alpha maps (Eq.~\ref{eq:render-final-c}).
Note that while we always render the feature image at $16^2$ during training, we can choose arbitrary resolutions at test time.

\figref{fig:disentanglement} suggests that our method disentangles objects from the background.
Note that this disentanglement emerges without any supervision, and the model learns to generate plausible backgrounds without ever having seen a pure background image, implicitly solving an inpainting task.
We further observe that our model correctly disentangles individual objects when trained on multi-object scenes with fixed or varying number of objects.
We further find that unsupervised disentanglement is a property of our model which emerges already at the very beginning of training (\figref{fig:training-progression}).
Note how our model synthesizes individual objects before spending capacity on representing the background.

\boldparagraph{Controllable Scene Generation}
As individual components of the scene are correctly disentangled, we analyze how well they can be controlled. 
More specifically, we are interested if individual objects can be rotated and translated, but also how well shape and appearance can be controlled.
In~\figref{fig:controllable-scene-gen}, we show examples in which we control the scene during image synthesis.
We rotate individual objects, translate them in 3D space, or change the camera elevation.
By modeling shape and appearance for each entity with a different latent code, we are further able to change the objects' appearances without altering their shape.

\boldparagraph{Generalization Beyond Training Data}
The learned compositional scene representations allow us to generalize outside the training distribution.
For example, we can increase the translation ranges of objects or add more objects than there were present in the training data (\figref{fig:generalization}).


\subsection{Comparison to Baseline Methods}\vspace{-0.12cm}
\begin{table}
  \centering
  \resizebox{1.\linewidth}{!}{
  \input{tables/table_64res.tex}}
  \vspaceundertab
  \caption{
      \textbf{Quantitative Comparison.}
      We report the FID score ($\downarrow$) at $64^2$ pixels for baselines and our method.
      }
  \label{tab:tab64}
\end{table}
\begin{table}
  \centering
  \resizebox{1.\linewidth}{!}{
  \input{tables/table_higheres.tex}}
  \vspaceundertab
  \caption{
    \textbf{Quantitative Comparison.}
    We report the FID score ($\downarrow$) at $256^2$ pixels for the strongest 3D-aware baselines and our method.
      }
  \label{tab:tab256}
\end{table}
\begin{figure}
  \centering
  \begin{subfigure}[t]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{gfx/experiments/cars/64/hologan/rotation}
    \includegraphics[width=\linewidth]{gfx/experiments/cars/256/hologan/rotation}\vspace{-0.1cm}
    \caption{$360^\circ$ Object Rotation for HoloGAN~\cite{Nguyen-Phuoc2019ICCV}}
  \end{subfigure}
  \begin{subfigure}[t]{\linewidth}
    \centering
  \includegraphics[width=\linewidth]{gfx/experiments/cars/64/graf/rotation_nocrop}
  \includegraphics[width=\linewidth]{gfx/experiments/cars/256/graf/rotation_nocrop}\vspace{-0.1cm}
  \caption{$360^\circ$ Object Rotation for GRAF~\cite{Schwarz2020NEURIPS}}
\end{subfigure}
  \begin{subfigure}[t]{\linewidth}
    \centering
  \includegraphics[width=\linewidth]{gfx/experiments/cars/64/ours/rotation_sm}
  \includegraphics[width=\linewidth]{gfx/experiments/cars/256/ours/rotation_2}\vspace{-0.1cm}
  \caption{$360^\circ$ Object Rotation for Our Method}
\end{subfigure}
\vspaceunderfig\vspace{-.1cm}
\caption{
  \textbf{Qualitative Comparison.}
      Compared to baseline methods, we achieve more consistent image synthesis for complex scenes with cluttered background at $64^2$ (top rows) and $256^2$ (bottom rows) pixel resolutions.
      Note that we disentangle the object from the background and are able to rotate only the object while keeping the background fixed.
      }
  \label{fig:qualitative-comparison}
\end{figure}
\begin{table}
    \center
    \resizebox{1.\linewidth}{!}{
    \input{tables/table_network_params.tex}}
    \vspace{-.23cm}
    \caption{
        \textbf{Network Parameter Comparison.}
        We report the number of generator network parameters in million.
    }
    \label{tab:netsize}
\end{table}
Comparing to baseline methods, our method achieves similar or better FID scores at both $64^2$~(\tabref{tab:tab64}) and $256^2$~(\tabref{tab:tab256}) pixel resolutions.
Qualitatively, we observe that while all approaches allow for controllable image synthesis on datasets of limited complexity, results are less consistent for the baseline methods on more complex scenes with cluttered backgrounds.
Further, our model disentangles the object from the background, such that we are able to control the object independent of the background (\figref{fig:qualitative-comparison}).

We further note that our model achieves similar or better FID scores than the ResNet-based 2D~GAN~\cite{Mescheder2018ICML} despite fewer network parameters ($0.41$m compared to $1.69$m).
This confirms our initial hypothesis that using a 3D representation as inductive bias results in better outputs.
Note that for fair comparison, we only report methods which are similar \wrt network size and training time (see~\tabref{tab:netsize}). %

\subsection{Ablation Studies}
\begin{table}
  \centering
  \resizebox{1.\linewidth}{!}{
  \input{tables/table_ablation_study.tex}}
  \vspaceundertab
  \caption{
      \textbf{Ablation Study.} 
      We report FID~($\downarrow$) on \textit{CompCars}
      without RGB~skip~connections (-Skip), without final activation (-Act.), with nearest neighbor instead of bilinear image upsampling (+ NN.\ RGB Up.), and with bilinear instead of nearest neighbor feature upsampling (+ Bi.\ Feat.\ Up.).
  }
  \label{tab:ablation-study}
\end{table}
\begin{figure}
  \centering
  \includegraphics[width=1.\linewidth]{gfx/experiments/church/256/ours/change_background}
  \includegraphics[width=1.\linewidth]{gfx/experiments/cars/256/ours/change_background}
  \vspace{-.3cm}
  \vspaceunderfig\vspace{-.1cm}
  \caption{
      \textbf{Neural Renderer.}
      We change the background while keeping the foreground object fixed for our method at $256^2$ pixel resolution.
      Note how the neural renderer realistically adapts the objects' appearances to the background.
      }
  \label{fig:neural-renderer}
\end{figure}
\begin{figure}
  \centering
  \begin{subfigure}[t]{1.\linewidth}
    \centering
  \includegraphics[width=1.\linewidth, trim= .3cm .5cm .3cm .0cm]{gfx/experiments/chairs/64/ours/canoncial_pose_0}
  \subcaption{$0^\circ$ Rotation for Axis-Aligned Positional Encoding~\cite{Mildenhall2020ECCV}}
\end{subfigure}
  \begin{subfigure}[t]{1.\linewidth}
    \centering
  \includegraphics[width=1.\linewidth, trim= .3cm .5cm .3cm .0cm]{gfx/experiments/chairs/64/ours/canoncial_pose_1}
    \subcaption{$0^\circ$ Rotation for Random Fourier Features~\cite{Tancik2020NEURIPS}}
\end{subfigure}
\vspaceunderfig\vspace{-.1cm}
  \caption{
      \textbf{Canonical Pose.}
        In contrast to random Fourier features~\cite{Tancik2020NEURIPS}, 
        axis-aligned positional encoding~\eqref{eq:pos-enc} encourages the model to learn objects in a canonical pose. %
      }
  \label{fig:canonical-pose}
\end{figure}
\vspace{-.13cm}\boldparagraphnovspace{Importance of Individual Components} The ablation study in~\tabref{tab:ablation-study} shows that our design choices of RGB skip connections, final activation function, and selected upsampling types improve results and lead to higher FID scores.

\boldparagraph{Effect of Neural Renderer}
A key difference to~\cite{Schwarz2020NEURIPS} is that we combine volume with neural rendering.
The quantitative~(\tabref{tab:tab64}~and~\ref{tab:tab256}) and qualitative comparisons~(\figref{fig:qualitative-comparison}) indicate that our approach leads to better results, in particular for complex, real-world data.
Our model is more expressive and can better handle the complexity of real scenes, \eg note how the neural renderer realistically adapts object appearances to the background (\figref{fig:neural-renderer}).
Further, we observe a rendering speed up: compared to~\cite{Schwarz2020NEURIPS}, total rendering time is reduced from $110.1$ms to $4.8$ms, and from $1595.0$ms to $5.9$ms for $64^2$ and $256^2$ pixels, respectively.

\boldparagraph{Positional Encoding} We use axis-aligned positional encoding for the input point and viewing direction (Eq.\ \ref{eq:pos-enc}). 
Surprisingly, this encourages the model to learn canoncial representations as it introduces a bias to align the object axes with highest symmetry with the canonical axes which allows the model to exploit object symmetry (\figref{fig:canonical-pose}).

\subsection{Limitations} 
\begin{figure}
  \centering
  \includegraphics[width=1.\linewidth]{gfx/experiments/celebA/256/ours/dataset_bias/rotation_0}
  \includegraphics[width=1.\linewidth]{gfx/experiments/celebA/256/ours/dataset_bias/rotation_1}
  \vspaceunderfigext
  \caption{
      \textbf{Dataset Bias.}
        Eye and hair rotation are examples for dataset biases: 
        They primarily face the camera, and our model tends to entangle them with the object rotation. %
      }
  \label{fig:dataset-bias}
\end{figure}
\vspace{-.12cm}\boldparagraphnovspace{Dataset Bias} Our method struggles to disentangle factors of variation if there is an inherent bias in the data.
We show an example in~\figref{fig:dataset-bias}: In the celebA-HQ dataset, the eye and hair orientation is predominantly pointing towards the camera, regardless of the face rotation.
When rotating the object, the eyes and hair in our generated images do not stay fixed but are adjusted to meet the dataset bias.

\boldparagraph{Object Transformation Distributions}
We sometimes observe disentanglement failures, \eg for \textit{Churches} where the background contains a church, or for \textit{CompCars} where the foreground contains background elements (see Sup.\ Mat.).
We attribute these to mismatches between the assumed uniform distributions over camera poses and object-level transformations and their real distributions.


==> stuff/table_ablation_study.tex <==
\begin{tabular}{c|cccc}
    \toprule
    Full  & -Skip & -Act.\ & +NN.\ RGB Up.\ & +Bi.\ Feat.\ Up.\ \\
    \midrule
    \textbf{16.16} & 16.66 &  21.61 & 17.28 & 20.68 \\
    \bottomrule
\end{tabular}

==> tables/refinement.tex <==

\begin{tabular}{lcc}
    \toprule
     & IoU  \\
    \midrule
    COCO  & 18  \\
    refined COCO  & 318  \\
    \bottomrule
\end{tabular}


==> tables/video_seg.tex <==

\begin{table}
  \centering
%   \resizebox{1.\linewidth}{!}{
 
\begin{tabular}{lcccc}
    \toprule
     & mIoU $\uparrow$ & Smoothness $\downarrow$ &  Inconsistency $\downarrow$  \\
    \midrule
    3DC-Seg  & \textbf{0.911} & NaN & NaN  \\
    Ours & 0.908 & \textbf{NaN} & \boldmath{NaN} \\
    \bottomrule
\end{tabular}

%   }

  \caption{
        Fine-tunning a video segmentation model using the consistency loss improves temporal consistency with a mild decrease in IoU (on DAVIS). 
      }
  \label{tab:video_seg}
\end{table}
